SAT-DIFF: A Tree Diffing Framework Using SAT Solving

Computing differences between tree-structured data is a critical but challenging problem in software analysis. In this paper, we propose a novel tree diffing approach called SatDiff, which reformulates the structural diffing problem into a MaxSAT problem. By encoding the necessary transformations from the source tree to the target tree, SatDiff generates correct, minimal, and type safe low-level edit scripts with formal guarantees. We then synthesize concise high-level edit scripts by effectively merging low-level edits in the appropriate topological order. Our empirical results demonstrate that SatDiff outperforms existing heuristic-based approaches by a significant margin in terms of conciseness while maintaining a reasonable runtime.

==> algo1.tex <==

\begin{comment}
    
\algtext*{EndWhile}% Remove "end while" text
\algtext*{EndIf}% Remove "end if" text
\algtext*{EndFor}
\algtext*{EndFunction}
\begin{algorithm}
\caption{Get Virtual Nodes}
\label{alg:get_virtual_nodes}
\begin{algorithmic}[]
\Function{GetTreeHistogram}{tree : Node, histogram : HashMap}
    \For{$\textbf{each}$ node $\textbf{in}$ tree}
        \State $id, label, type, value \gets \text{node.get\_node\_info()}$
            \State $histogram[(label, type, value)].increment()$
    \EndFor
    \State \textbf{return} histogram
\EndFunction
\State
\Function{GetVirtualNodes}{src\_tree: Node, trg\_tree: Node}
    \State $src\_node\_histogram \gets \text{GetTreeHistogram}(src\_tree, HashMap(default\_value=0))$
    \State $trg\_node\_histogram \gets  \text{GetTreeHistogram}(trg\_tree, HashMap(default\_value=0))$
    \State $virtual\_nodes \gets []$
    \For{$(label, type, value)$ $\textbf{in}$ $\text{trg\_node\_count\_dict.keys()}$}
        \State $diff$ $\gets$ $trg\_node\_histogram [(label, type, value)]$ $-$ $src\_node\_histogram[(label, type, value)]$
        \If{$diff > 0$}
            \State $unique\_ids \gets \text{Generate\_Unique\_Ids(num = diff)}$
            \State $virtual\_nodes.\text{append}(\text{Generate\_Nodes}(unique\_ids, (label, type, value)))$
        \EndIf
        
    \EndFor
    \State \textbf{return} virtual\_nodes
\EndFunction
\end{algorithmic}
\end{algorithm}

\end{comment}


\begin{minipage}{0.55\textwidth}
% \vspace{-0.2cm}
\begin{algorithm2e}[H]
    \caption{Get Virtual Nodes}
    \label{alg:get_virtual_nodes}
    \small
    \DontPrintSemicolon
    % \SetKwInOut{KwIn}{myinput }
    % \SetKwInOut{Param}{Parameterxxxxx}
    \SetKwProg{Fn}{Function}{}{end}
    \SetKwFunction{getV}{GetVirtualNode}
    % \SetKwFunction{Fget}{GetTreeHistogram}

    \KwIn{source tree($s$), target tree($t$)}
    \KwOut{a set of valid virtual nodes($vns$)}
    % \Param{neural embedding \texttt{embed}, proof grammar $G$}

    % \Fn{ \Fget{source\_tree, target\_tree} }{
    %     \For{$\textbf{each}$ node $\textbf{in}$ tree} {
    %         % $id, label, type, value \gets \text{node.get\_node\_info()}$ \;
    %         $histogram[node.(label, type, value)].increment()$ \;
    %     }
    %     \Return{histogram}
    % }

    \Fn{ \getV{s, t} }{
        % $src\_node\_histogram$ $\gets$ \text{GetTreeHistogram}(source\_tree, HashMap(default\_value=0))\;
        % $s\_histogram$ $\gets$ Histogram(key: n.(label, type, value), value: $\#(n') \in$ $\textit{s}$, s.t. n' $\leftrightarrow$ n)\;
        $s\_hist$ $\gets$ Histogram([ $n$.(label, value) $\textit{for}$ $n \in$ $\textit{s}$])\;
        % $trg\_node\_histogram$ $\gets$  \text{GetTreeHistogram}(target\_tree, HashMap(default\_value=0)) \;
        % $t\_histogram$ $\gets$ Histogram(key: n.(label, type, value), value: $\#(n') \in$ $\textit{t}$, s.t. n' $\leftrightarrow$ n)\;
        $t\_hist$ $\gets$ Histogram([ $n$.(label, value) $\textit{for}$ $n \in$ $\textit{t}$])\;
        % $trg\_node\_histogram
        $vns \gets []$ \;

        \For{$attrs$  $\textbf{in}$ \text{t\_hist.keys()}}{
            \textit{diff} $\gets$ $\text{t\_hist} [attrs] - \text{s\_hist[$attrs$}]$

            \If{diff > 0}{
                % $unique\_ids \gets \text{Generate\_Unique\_Ids}(num = diff)$ \;
                $vns.\text{append}(\text{Generate\_Nodes}(
                \newline attrs, num\_unique\_copies=\textit{diff}))$                 
            }
        }
        \Return{vns}
}      
\end{algorithm2e} 
\end{minipage}%
\hspace{0.3cm}
\begin{minipage}{0.43\textwidth}
% \vspace{-1cm}
\begin{algorithm2e}[H]
    \caption{Extract Potential Edges}
    \label{alg:get_pot_edges}
    \small
    \DontPrintSemicolon
    % \SetKwInOut{KwIn}{myinput }
    \SetKwProg{Fn}{Function}{}{end}
    \KwIn{source tree\ ($s$),\ target tree\ ($t$)}
    \KwOut{a set of potential edges(\textit{p})}
    \SetKwFunction{getpot}{ExtractPotentialEdges}
    % \SetKwFunction{getinfo}{ExtractTypeInfo}
    
    % \Fn {\getinfo{$target\_tree$}}{
    % $ps \leftarrow empty \text{ Set()}$  \tcp*[l]{parent edge info}
    % \For{\textbf{each} Edge(p, $k^{th}$, c) in target\_tree}{
    %     % Edge(parent,$k^{th}$,child)
    %     % p, k, c \leftarrow e

    %     ps $\cup$ {(p.label, p.type, p.value),$k^{th}$,(c.label,c.type,c.value)} 
        
    %     % $\text{add}((p.label, p.type, p.value),k^{th},(c.label,c.type,c.value)) \textbf{to } Set $
    % }   
    % \Return{ps}  
    % }  

    \Fn{\getpot{$s$, $t$}}{
    % $virtual\_nodes \gets \text{GetVirtualNodes}(s, t)$ \;

    $src\_space \gets s \cup \text{GetVirtualNodes}(s, t)$ \;

    $ p \gets [] $ \;
    
    \For{$\textbf{each}$ unconnected $e$ \textbf{in} t}{
    % \If{$((p.(label, type, value)), k^{th}, (c.(label, type, value))) \in edge\_type\_info$ }
    \lIf{ $e$' $\in$ $src\_space$ $and$ e  $\leftrightarrow$ $e$'}
    {p.append(e)}
    }
    \Return{p}
    }
\end{algorithm2e}
\end{minipage}




% \tcc{xxx} // in a separate line, /* xxx */
% \tcp*[l]{xxx}  // immediately next to the statement
% \tcp*{} // insert spaces so that the comment is at the rightmost    



% \begin{algorithm2e}
%     \DontPrintSemicolon
%     % \SetKwInOut{KwIn}{myinput }
%     \SetKwProg{Fn}{Function}{}{end}

%     \caption{Get Type Info}
%     \label{alg:get_type_nodes}
%     \KwIn{target\_tree $T$}
%     \KwOut{all child information of $T$}
%     \SetKwFunction{getinfo}{GetTypeInfo}
    
%     \Fn {\getinfo{$T$}}{
%     $ps \leftarrow empty \text{ Set()}$  \tcp*[l]{parent edge info}
%     \For{each Edge(p, $k^{th}$, c) in target\_tree}{
%         % Edge(parent,$k^{th}$,child)
%         % p, k, c \leftarrow e

%         ps.insert( (p.label, p.type, p.value),$k^{th}$,(c.label,c.type,c.value) ) 
        
%         % $\text{add}((p.label, p.type, p.value),k^{th},(c.label,c.type,c.value)) \textbf{to } Set $
%     }   
%     \Return{ps}  
%     }  
% \end{algorithm2e}




% \begin{algorithm2e}
%     \caption{Synthesizing high-level edit action}
%     \label{alg:synth}

%     \DontPrintSemicolon
%     % \SetKwInOut{KwIn}{myinput }
%     \SetKwProg{Fn}{Function}{}{end}
%     \SetKwFunction{Synth}{Synthesizing}

%     \KwIn{disconnections, deletions, connections}
%     \KwOut{high-level Op}

%     \Fn{\Synth{disconnections, deletions, connections}}{
%     $updates \gets$ [] \;
%     $moves \gets []$ \;
%     \While{True}{
%     \For {any pair of (con,del)}{
%     \If{($con.p == del.p)$ \textbf{and} $(con.k^{th} value == del.k^{th} value$)}{
%         Remove con and del \;
%         $update \gets$ $p, con.k^{th}, c$\;
%         $updates.insert(update)$ \;
%     }
%     }
%     \For{each $k^{th}$ grandchild of del.node}{
%     \If{grandchild is moved to be the $k^{th}$ child of con.c}{
%         ignore this move because its relative position in the tree does not change \;
%     } \EIf{grandchild is unmatched}{
%         $child\_management \gets del.child\_node$, $k^{th}$, $grandchild$ \;
%     }
%     }
%     }

% \end{algorithm2e}

==> algo2.tex <==
% \begin{algorithm}
% \caption{Get Potential Edges}
% \label{alg:get_potential_edges}
% \begin{algorithmic}[]
% \Function{GetTypeInfo}{target\_tree : Node}
%     \State $parent\_edge\_info \gets \text{empty Set()}$
%     \For{$\textbf{every}$ Edge(parent, k\_th, child) $\textbf{in}$ target\_tree}
%         \State \textbf{add} $((\text{parent.label},\text{parent.type}, \text{parent.v}), k\_th, (\text{child.label},\text{child.type}, \text{child.value}))$ \textbf{to} $\text{Set}$
%     \EndFor
%     \State \textbf{return} parent\_edge\_info
% \EndFunction
% \State
% \Function{GetPotentialEdges}{source\_tree: Node, target\_tree: Node}
%     \State $virtual\_nodes \gets GetVirtualNodes(source\_tree, target\_tree)$
%     \State $source\_space \gets Merge(source\_tree, virtual\_nodes)$
%     \State $parent\_edge\_info \gets \text{GetTypeInfo}(target\_tree)$
%     \State $potential\_edges \gets []$
%     \For{$\textbf{every unconnected}$ Edge(parent, k\_th, child) $\textbf{in}$ source\_space}
%         \If{$((\text{parent.(label, type, value)}), k\_th, (\text{child.(label, type, value)})) \in \text{parent\_edge\_info}$}
%             \State \textbf{add} Edge(parent, k\_th, child) \textbf{to} $\text{potential\_edges}$
%         \EndIf
%     \EndFor
%     \State \textbf{return} potential\_edges
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

% \begin{minipage}{0.5\textwidth}
% \begin{algorithm2e}
%     \caption{Extract Potential Edges}
%     \label{alg:get_pot_edges}
%     \DontPrintSemicolon
%     % \SetKwInOut{KwIn}{myinput }
%     \SetKwProg{Fn}{Function}{}{end}
%     \KwIn{source tree\ ($s$),\ target tree\ ($t$)}
%     \KwOut{a set of potential edges(\textit{p})}
%     \SetKwFunction{getpot}{ExtractPotentialEdges}
%     % \SetKwFunction{getinfo}{ExtractTypeInfo}
    
%     % \Fn {\getinfo{$target\_tree$}}{
%     % $ps \leftarrow empty \text{ Set()}$  \tcp*[l]{parent edge info}
%     % \For{\textbf{each} Edge(p, $k^{th}$, c) in target\_tree}{
%     %     % Edge(parent,$k^{th}$,child)
%     %     % p, k, c \leftarrow e

%     %     ps $\cup$ {(p.label, p.type, p.value),$k^{th}$,(c.label,c.type,c.value)} 
        
%     %     % $\text{add}((p.label, p.type, p.value),k^{th},(c.label,c.type,c.value)) \textbf{to } Set $
%     % }   
%     % \Return{ps}  
%     % }  

%     \Fn{\getpot{$s$, $t$}}{
%     % $virtual\_nodes \gets \text{GetVirtualNodes}(s, t)$ \;

%     $source\_space \gets s \cup \text{GetVirtualNodes}(s, t)$ \;

%     $ p \gets [] $ \;
    
%     \For{$\textbf{each}$ unconnected $e$ \textbf{in} target\_space}{
%     % \If{$((p.(label, type, value)), k^{th}, (c.(label, type, value))) \in edge\_type\_info$ }
%     \lIf{ $e$' $\in$ $source\_space$ $and$ e  $\leftrightarrow$ $e$',}
%     {p.append(e)}
%     }
%     \Return{p}
%     }

% \end{algorithm2e}
% \end{minipage}

==> algo3.tex <==
% def sythesize(disconnections, deletions, connections):
%     updates, moves <- [], []
%     for (del, con) in deletions, connections :
%         if (del. k^{th} == con.k^{th}) and (del.parent == con.parent):
%             remove



\begin{algorithm2e}
    \caption{synthesizing high-level edit script}
    \label{alg:synth}
    \DontPrintSemicolon
    % \SetKwInOut{KwIn}{myinput }
    \SetKwProg{Fn}{Function}{}{end}
    \SetKwFunction{Synth}{synthesizing}
    \SetKwFunction{rep}{replace\_node}

    \KwIn{dependency graph(List[\textit{dpg}])}
    \KwOut{high-level edit actions(\textit{dpg})} \;


    \Fn{\rep{graph,n,ls}}{
    \For{n' in ls}{
    \For{nn in n'.neighbors}{
    graph.delete\_edge(n', nn) \;
    graph.add\_edge(n,nn) \;
    }
    }
    } \;

    \Fn{\Synth{dpg}}{
    \For{graph in dpg}{
    moves = new Hashmap() \;
    \For{op in graph}{
    \If{con(p,k,node) and dis(p',$k_2$,node) in {op} $\cup$ op.neighbors}{
    con, dis = com(p, k, node), dis(p', $k_2$, node) \;
    \If{p' in moves}{
    new\_op = moves[p'] \;
    swp = Swp(node, node') \;
    \texttt{replace\_node}(graph, swp, [con, dis, moves[p']])
    }
    \Else{mov = Mov(p', $k_2$, node, p, $k_1$) \;
    \texttt{replace\_node}(graph, mov, [con, dis]) \;    
    % \If{moves[p].is\_empty}{ moves[p] = [mov]
    % } \Else{moves[p].append([mov])}
    
    moves[p] = [mov] \textbf{if} moves[p].is\_empty \textbf{else} moves[p].append([mov])}
    }\ElseIf{del(p, k, node) and con(p, k, vn) in {op} $\cup$ op.neighbors}{
    upd = Upd(node\_vn) \;
    replace\_node(graph, upd, [del, con])
    }
    }
    }
    }

    \tcc{The other connections and deletions are automatically considered to be Ins and Del}



    % \Fn{\Synth{dpg}}{
    % % $vns \gets$ GetVirtualNodes(s, t) \;
    % $visited \gets Set()$\;
    % \For {unvisited {action}, $\textit{a}$, $\in$ dpg}{
    % % $visited.add(action)$\;
    % $stack \gets [a]$\;
    % \While{stack contains unvisited actions}{
    % % curr $\gets$ stack.pop()\;
    % action $\gets$ stack.pop()\;
    % $visited$.add(action)\;
    % stack.extend( [action's unvisited neighbors in \textit{dpg}] ) \;
    % \lIf{pattern of \ $\texttt{Mov}$ $\in$ action.neighbors}{replace the pattern with $\texttt{Mov}$}
    % \lIf{pattern of \ $\texttt{Swp} \in$ action.neighbors}{replace the pattern with $\texttt{Swp}$}
    % \If{pattern of \ $\Upd{n}{i}{n'} \in $ action.neighbors}{
    %     replace the pattern with $\Upd{n}{i}{n'}$\;
    %     \For{\textbf{each} $k^{th}$ $nn$ $\in$ $n'$.neighbors}{\lIf{$\Mov{nn}{n}{i}{n'}{i} \in nn$'.neighbors}{remove it from $dpg$} 
    %     %  pattern in $n'$.neighbors
    %     \If{$\texttt{Upd}$ does not depend on any action of $nn$}
    %     {insert \{$\texttt{Upd}$ $\rightarrow$ $\del{n'}{k}{nn}$\} in \textit{dpg}\;
    %     }
    %     }       
    % }
    % }
    % }    
    % \tcc{Treat the $\texttt{del}$'s and $\texttt{con}$'s left in $dpg$ as $\texttt{Del}$'s and $\texttt{Ins}$'s}
    % \Return{\textit{dpg}}   
    % }
\end{algorithm2e}


% \If{($con.p == del.p)$ \textbf{and} $(con.k^{th} == del.k^{th}$) \textbf{and} $con.c \in vns$}{
    %     Remove con and del from Cons.$remove$(con), Dels\;
    %     % $update \gets$ $$\;
    %     $updates.append((con.p, con.k^{th}, con.c))$ \;
    % }
    
    % \For{each $k^{th}$ grandchild of del.c}{
    % \If{(con.c, $k^{th}$, grandchild) $\in$ moves}{
    %     remove this move from \textit{moves}\;
    %     \tcp{its relative position in the tree does not change }
    % } 
    % \If{grandchild is unmatched}{
    %     $child\_management \gets del.c,$ $k^{th}$, grandchild \;
    %     $deletions.append(child\_management)$ \;
    % }
    % }
    % \lIf{no update detects in this iteration}{$\textit{break}$\;}
    % }
    % \For{each pair of (con, dcon) in connections, disconnections}{
    %     \If{con.c == dcon.c}{
    %     remove con, dcon from their sets\;
    %     % move $\gets$ (con.p, $con.k^{th}$, dcon.c)\;
    %     $\textit{moves}.append$((con.p, $con.k^{th}$, dcon.c))\;
    %     }
    % }
    % \Return $\textit{updates}, \textit{moves}, \textit{deletions}, \textit{connections}$

==> algo_overview.tex <==
\begin{minipage}{0.43\textwidth}
% \vspace{-1cm}
\begin{algorithm2e}[H]
    \caption{Extract Potential Edges}
    \label{alg:get_pot_edges}
    \small
    \DontPrintSemicolon
    % \SetKwInOut{KwIn}{myinput }
    \SetKwProg{Fn}{Function}{}{end}
    \KwIn{source tree\ ($s$),\ target tree\ ($t$)}
    \KwOut{a set of potential edges(\textit{p})}
    \SetKwFunction{getpot}{ExtractPotentialEdges}
    % \SetKwFunction{getinfo}{ExtractTypeInfo}
    
    % \Fn {\getinfo{$target\_tree$}}{
    % $ps \leftarrow empty \text{ Set()}$  \tcp*[l]{parent edge info}
    % \For{\textbf{each} Edge(p, $k^{th}$, c) in target\_tree}{
    %     % Edge(parent,$k^{th}$,child)
    %     % p, k, c \leftarrow e

    %     ps $\cup$ {(p.label, p.type, p.value),$k^{th}$,(c.label,c.type,c.value)} 
        
    %     % $\text{add}((p.label, p.type, p.value),k^{th},(c.label,c.type,c.value)) \textbf{to } Set $
    % }   
    % \Return{ps}  
    % }  

    \Fn{\getpot{$s$, $t$}}{

    $src\_space \gets s \cup \text{GetVirtualNodes}(s, t)$ \;

    $ p \gets [] $ \;
    
    \For{$\textbf{each}$ unconnected $e$ \textbf{in} t}{
    \lIf{ $e$' $\in$ $src\_space$ $and$ e  $\leftrightarrow$ $e$'}
    {p.append(e)}
    }
    \Return{p}
    }
\end{algorithm2e}
\end{minipage}

==> intro_1.tex <==
\section{Introduction}
\label{sec:intro}


\allen{The paper does not compare against the standard version of Gumtree, but does not disclose this. Choosing a different implementation either needs to be motivated, or the work should be compared to the real implementation.}



\allen{The chosen measure of optimality also needs to be motivated, either by a downstream application or by evaluating the human-readability of the results.}


\allen{Moreover, the implications of the specific form of optimality chosen by this work need to be better explained to the reader.}


Software systems need to undergo evolution to fulfill their intended objectives, thereby contributing to the emergence of the field known as \emph{software evolution analysis} \cite{SoftwareEvolution}.
One of the most fundamental problems in software evolution analysis is \emph{source code differencing}, which has wide applications in version control systems, program analysis, and debugging. The problem involves computing the differences between two distinct source code files and determining the transformation from one to the other through a series of edit actions, commonly referred to as \textit{edit scripts}. In typical software development environments, edit scripts are computed between different versions of the same code file to understand changes applied to the original code file.


Viewing code as text is a straightforward approach for computing edit scripts. For instance, when given two versions of a source code file, the Unix {\fontfamily{cmss}\selectfont diff} tool utilizes the Myers algorithm \cite{DBLP:journals/algorithmica/Meyers86} at the text level of granularity to generate an edit scripts that identifies added or deleted lines. However, edit scripts generated by tools like Unix {\fontfamily{cmss}\selectfont diff} and other text-level methods can often be challenging for users to interpret. These methods do not take the structure of the code into account, thereby necessitating further analysis in order to understand the intention behind code changes.

To address this issue, a line of work has emerged that computes edit scripts at the abstract syntax tree (AST) level of granularity. This is also known as the \emph{tree/structural differencing problem}. By incorporating the structural information of the code, computing tree diffing edit scripts can significantly improve the alignment of programmers' intentions, enabling high-level edit operations such as \textit{update}, \textit{move}, \textit{insert}, and \textit{delete}. The most widely adopted approach for computing tree diffing involves addressing two main sub-problems: 1) identifying a suitable matching between the source and target trees, and 2) deducing an edit script based on the established matching \cite{ChawatheRGW96}. However, it is worth noting that finding the optimal or minimum tree-differencing edit script has been proven to be NP-hard \cite{DBLP:journals/tcs/Bille05}. Consequently, most existing methods rely on heuristics to search for good matching and deduce plausible edit scripts, thus usually failing to yield optimal solutions.

In this paper, our objective is to compute optimal edit scripts between two code trees while providing a formal guarantee of optimality. Our approach, known as {\satdiff}, can be broken down into three distinct phases. First and foremost, rather than focusing on optimizing the heuristics utilized in previous approaches to achieve a good matching, we adopt an orthogonal approach. Specifically, we reframe the tree diffing problem as a maximum satisfiability {\maxsat} problem \cite{stutzle2001review} and leverage state-of-art solvers to efficiently search for the optimal edits to be applied to the source tree while ensuring it becomes isomorphic to the target tree. At the heart of {\satdiff} is a collection of soft and hard constraints, which not only guarantee the correctness of the discovered solution but also facilitate the deduction of an optimal and type safe edit script. Our intuition behind {\satdiff} is rather straightforward: we utilize a solver that is specifically designed for solving NP problems to tackle the inherent NP complexity of the matching problem itself. While solving computationally expensive NP problems like tree matching can often result in significant computational costs, it is important to note that recent advancements in solvers, coupled with our own optimizations, have made it feasible to obtain timely results. In fact, the running time of our approach is on par with that of heuristic-based approaches, as we will demonstrate in our experimental section. 

% The conciseness of our edit scripts ensures that edit actions are exclusively applied to nodes or subtrees that undergo changes, effectively excluding any irrelevant nodes and subtrees. This focus on capturing only the necessary modifications contributes to the overall efficiency and clarity of the edit scripts.


Secondly, we deduce the solution returned by the {\maxsat} solver into a low-level edit script --- a sequence of simple atomic edit actions. Those atomic actions not only directly align with our SAT encoding constraints but also can be naturally composed into intuitive high-level edit actions such as \texttt{Upd} and \texttt{Mov}. It is worth highlighting that the solver's output of node matching and low-level edit scripts achieves both correctness and optimality, thanks to our carefully designed encoding constraints. In addition, our constraints facilitate several other notable features of deduced edit scripts, such as \emph{type safe editing} \cite{truediff}. The type safety property ensures that all intermediate trees, following each atomic edit action, remain well-typed, even if they may contain holes. The type safety guarantee in our approach is a notable advantage that is rarely found in previous approaches, such as \textit{Gumtree} \cite{gumtree}. We further elaborate on the semantic meaning and type system of our edit actions, and provide formal proofs of the correctness, optimality, and type safety of our low-level edit scripts.


% In the {\fontfamily{cmss}\selectfont GumTree} framework, for example, an insert action can easily violate a function signature by adding an additional child beyond the allowed limit. Whereas our {\satdiff} enforces the correct number of children for internal nodes through our hard constraints. In addition, our encoding constraints further ensure that the type of children for a parent node remains consistent, which goes beyond the level of guarantee provided by previous type-safe tree diffing approaches \cite{truediff,hdiff,DBLP:conf/icfp/LempsinkLL09}. 


% Our experimental results demonstrate {\satdiff} outperforms existing type-safe approaches in terms of the conciseness and optimality of edit scripts.

% In addition to its advancements in type-safety, our approach outperforms existing type-safe approaches in terms of the conciseness and optimality of the generated edit scripts. This superiority is demonstrated in the experimental section of our study, where we provide empirical evidence of the improved performance and effectiveness of our approach.


In the final step, we transform the low-level edit scripts into high-level edit scripts, presenting them in a more intuitive and user-friendly format for end users. This transformation is achieved through an efficient algorithm that synthesizes atomic edit actions into cohesive high-level edit actions, taking into account an appropriate execution order. Rather than directly utilizing the commonly used edit actions introduced in previous work, we redefine and expand these actions to enhance the type safety, and expressiveness of our edit scripts. For example, in the approach introduced by Chawathe et al., the \textit{delete} action is limited to deleting a single node, requiring multiple \textit{delete} actions to delete a subtree within the edit script. In contrast, our \texttt{del} action enables the direct deletion of a subtree, significantly simplifying the edit script's size. Our synthesizing approach allows high-level edit scripts to inherit several intriguing features from low-level edit scripts, including type safety. We further elaborate on the semantic meaning and type system of our edit actions, as well as some formal guarantees on the resulting edit script.
Our experimental results also suggest our generated high-level edit scripts outperform existing approaches in terms of conciseness.

% By leveraging our proposed edit actions in conjunction with the {\fontfamily{cmss}\selectfont merge} algorithm, we inherit several intriguing features from the low-level edit scripts, including type-safety. 
% We further elaborate on the semantic meaning and type system of our edit actions, and provide a formal proof of the correctness and type-safety of the resulting edit script.


% Our proposed framework, called {\satdiff}, utilizes a {\Large S}AT solver to facilitate the search for the optimal solution. At the core of {\satdiff} is the design of constraints, which enables state-of-the-art  {\Large M}AX{\Large S}AT solvers to efficiently identify the optimal solution. We create two sets of constraints for the nodes and edges of the two trees being compared. One set of constraints is hard and thus cannot be violated. This guarantees the validity of the edit scripts, ensuring that the source tree is exactly reconstructed in the target space. The other set of constraints is soft, meaning they can be violated if needed. Violating such constraints facilitates the reconstruction of the source tree. By solving this  {\Large M}AX{\Large S}AT problem, we obtain the least set of soft constraints that need to be violated, which are then interpreted as a sequence of edit operations. Like most AST-based code differencing methods, {\satdiff} supports the four standard edit operations, including "update," "move," "insert," and "delete". 

% To enable our proposed framework to be language-agnostic, we design a reduced tree format that can be agreed upon by different formats of the abstract syntax tree. This format is intended to extract the essential structural information from the original AST while maintaining a high degree of simplicity and efficiency. By reducing the AST to this common format, we can compare trees from different programming languages using the same set of constraints and operations. This is particularly useful in our framework as it allows us to focus on the tree-differencing problem without being burdened by language-specific syntax details. We also introduce some optimization techniques for the design of the reduced tree format as well as constraints, which efficiently speed up the search process of the  {\Large M}AX{\Large S}AT solver. We will provide more technical details in the remaining paper. 


% While the NP-hard nature of the problem may raise performance concerns, our empirical results suggest that {\satdiff} performs comparably to state-of-the-art heuristic-based approaches in most cases in terms of running time. Moreover, {\satdiff} generally outperforms other approaches in terms of generating the minimum edit scripts, making it appealing in many real-world applications. While user-defined instructions are not easily incorporated into existing approaches, {\satdiff} can easily support a wide range of instructions from users due to its nature of solving an {\Large S}AT problem. Based on these merits, we believe that {\satdiff} has the potential to be a more reliable and user-friendly tool for source coding/tree differencing. We provide further details on our approach in the following sections. In addition, {\satdiff} allows additional user-defined constraints for solving minimum edit scripts which are not well-supported in most existing methods.


In summary, we make the following contributions:
\begin{itemize}
    \item We present a novel approach --- {\satdiff} for tree/structure diffing by formulating the problem as a {\maxsat} problem. By leveraging state-of-the-art solvers, we can efficiently find the optimal solution, which existing heuristic-based methods often struggle with.
    \item We meticulously design a comprehensive collection of soft and hard constraints that facilitate the derivation of correct, optimal, and type-safe edit scripts. 
    \item We propose efficient algorithms for converting {\Large S}AT solutions into edit scripts, which are composed of concise yet expressive edit actions.
    \item We present the semantics and type system of our defined edit actions, along with formal proofs of correctness, optimality, and type-safety for the generated edit scripts.
    \item Our empirical results indicate that {\satdiff} outperforms existing approaches, such as \textit{Gumtree} and \textit{truediff}, on a real-world benchmark. Additionally, {\satdiff} demonstrates comparable running times to heuristic-based approaches.
\end{itemize}

==> overview_1.tex <==
% \begin{figure}[h]
%     \centering
%     \includegraphics[page=3, width=0.9\textwidth,trim={0 4.5cm 0 5cm}, clip]{figures/sat_diff.pdf}
%     \caption{Overview of the {\satdiff} Algorithm.}
%     \label{fig:{\satdiff}}
% \end{figure}

\section{Overview of {\satdiff}}
\label{sec:overview}

In this section, we provide an overview of our {\satdiff} framework, a novel approach to tree diffing using the {\maxsat} solver. The {\satdiff} framework takes a pair of source and target code files written in a specific programming language as input and generates an edit script that transforms the source tree into the target tree. The {\satdiff} framework consists of four key phases, which are illustrated as follows.

\textbf{The parsing phase} This phase involves taking a pair of source and target code files written in a specific programming language and parsing them into the source AST $T$ and the target AST $T'$. To give a concrete example, let's consider the following pair of codes:
\begin{align*}
&Source:
Sub( Add( A, (Mul( B, C) ), Sub( Sub( D, Sub( E, F) ) ) )) \\
&Target:
Sub( Add( G, Add( B, C) ), Sub( D, A)) 
\end{align*}
which are parsed into tree-structured data or an Abstract Syntax Tree (AST), as illustrated in Figure \ref{fig:overview_sat1}. Each node in the tree is assigned a unique identifier, allowing for easy referencing of individual nodes.
The parsing phase is a standard step in almost every tree/structural diffing approach, so we won't delve into it extensively.


% The encoding phase serves as the fundamental component of {\satdiff}. Its primary purpose is to convert the tree diffing problem into a {\Large M}AX{\Large S}AT problem, offering the flexibility to define specific solution requirements through the design and imposition of both hard and soft constraints.


% \begin{figure}
%     \centering
%     \includegraphics[page=2, trim={0.6cm 0 0.5cm 0}, clip]{figures/overview_popl.pdf}
%     \caption{Overview of the {\satdiff} Algorithm.}
%     \label{fig:overview_sat}
% \end{figure}

\begin{figure}
    % \vspace{-5pt}
    \centering
    \subfloat[Parsing phase]{
    \centering
            \includegraphics[page=2, width=0.3\textwidth,trim={0cm 0.5cm 23cm 0.5cm}, clip]{figures/overview_popl.pdf}
            \label{fig:overview_sat1}
        }
    \subfloat[Encoding phase]{
    \centering
            \includegraphics[page=2, width=0.31\textwidth,trim={11cm 0.5cm 11.8cm 0.5cm}, clip]{figures/overview_popl.pdf}
            \label{fig:overview_sat2}
        }
    \subfloat[Deducing and synthesizing phase]{
    \centering
            \includegraphics[page=2, width=0.33\textwidth, trim={22.2cm 0.5cm 0cm 0.5cm}, clip]{figures/overview_popl.pdf}
            \label{fig:overview_sat3}
        }   
    \caption{Overview of the {\satdiff} Algorithm.}
    \label{fig:overview_sat}
\end{figure}




\textbf{The encoding phase} In this phase, we first generate a set of propositional Boolean variables to encode the states of edges and the matching between nodes from both the target tree $T'$ and the source tree $T$. To be more specific, we use a variable $\evar{n}{i}{n_c}$ to indicate whether the $i$\textsuperscript{th} edge $e_i$ of node \nd{n} is connected to \nd{n_c}. For instance, $\evar{2}{1}{4}$ encodes the usage of the first edge of the node \nd{2} to \nd{4} in our example. The literal $\evar{n}{i}{n_c}$ indicates that the edge $e_i$ is being utilized, signifying a connection between the corresponding nodes \nd{n} and \nd{n_c}. On the other hand, the negation $\negevar{n}{i}{n_c}$ indicates that the edge $e_i$ is not being used, nodes $n$ and $n_c$ may be disconnected or connected through other edges. It is important to note that the edge $(n,e_i)$ represents the $i$\textsuperscript{th} child position of the parent node ($n$), and the number of allowable edges is determined by the type/signature of $n$. 

Similarly, a variable $\mvar{n}{n'}$ encodes the usage of a match between a node $n$ from the source tree $T$ and a node $n'$ from the target tree $T'$. The literal $\mvar{n}{n'}$ indicates that the match between $n$ and $n'$ is established, while the negation $\negmvar{n}{n'}$ indicates that there is no match between $n$ and $n'$. Note that a node $n$ may have more than one potential matching node in $T'$, thus will create a number of match variables for node $n$, but only one of them will be used. 
For instance, node 1 has two potential matchings (node 12 and 14) in our cases, which are encoded using $\mvar{1}{12}$
and $\mvar{1}{14}$.

% The subsequent step involves encoding a set of hard and soft constraints to address the tree-diffing problem. To provide a conceptual understanding, let's envision a source space comprising the source tree $T$ along with \emph{virtual nodes} --- additional nodes from the target tree $T'$ that do not exist in $T$ (without any edges), as shown in Figure \ref{fig:iso_exmaple1}. By manipulating the connections between nodes in the source space, such as disconnecting or connecting specific edges, it becomes possible to find a tree within the source space that is isomorphic to the target tree, as illustrated in Figure \ref{fig:iso_exmaple}. Isomorphism implies that the two trees are identical in structure except for differences in node identifiers.

The subsequent step involves encoding a set of hard and soft constraints to address the tree-diffing problem. To provide a conceptual understanding, let's envision a source space comprising the source tree $T$ along with \emph{virtual nodes} --- additional nodes from the target tree $T'$ that do not exist in $T$. In Figure \ref{fig:iso_exmaple1}, nodes 21 and 22 are examples of such virtual nodes. By manipulating the connections between nodes in the source space, such as disconnecting or connecting specific edges, it becomes possible to find a tree within the source space that is isomorphic to the target tree, as illustrated in Figure \ref{fig:iso_exmaple}. Isomorphism implies that the two trees are identical in structure except for differences in node identifiers.

It is worth noting that except existing edges are being encoded, potential edges (currently not existing) are also encoded. So a truth assignment to the edge variables essentially serves to manipulate connections between nodes through existing and potential edges. In addition to this, the match variables, in conjunction with the edge variables, are employed to encode a set of indispensable requirements using hard constraints to ensure the validity of solutions. These constraints, include but are not limited to: 1) a child has only one parent, and 2) local structure must be matched. For instance, the hard constraint for matching local structures ensures the following: If nodes $n_1$ and $n_2$ in the source tree $T$ are matched with nodes $n_1'$ and $n_2'$ in the target tree $T'$ (indicated by the truth values 
$\mvar{n_1}{n_1'}$ and $\mvar{n_2}{n_2'}$
being true), and if $n_1'$ and $n_2'$ are connected through edge $e_1$, then it is mandatory that $n_1$ and $n_2$ are connected through the corresponding edge $e_1$ (indicated by $\evar{n_1}{1}{n_2}$
being true).


Finally, we incorporate a soft constraint that pertains to the usage of existing and potential edges. These soft constraints specify that both disconnecting existing edges and adding new edges should incur a certain cost. And the main objective of the solver is to minimize the total cost associated with such edge modifications. Intuitively, these soft constraints incentivize the solver to make minimal changes to the structure of the source tree, ultimately contributing to the optimality of the derived edit script. Further details regarding the design of these propositional Boolean variables and constraints will be discussed in Section \ref{sec:phase1}.

% prioritize the utilization of non-existing edges over modifying the existing ones. This emphasis on utilizing non-existing edges 

% ultimately contributes to the optimality of the discovered edit script. Further details regarding the design of these propositional Boolean variables and constraints will be discussed in Section \ref{sec:phase1}.




\begin{figure}
    \centering
    \subfloat[Source space]{
    \includegraphics[page=3, width=0.53\textwidth, trim={0 5cm 15cm 3cm}, clip]{figures/diff_exm.pdf}
    \label{fig:iso_exmaple1}
    }  
    \subfloat[Target tree]{
    \includegraphics[page=3, width=0.42\textwidth, trim={19cm 5cm 0.3cm 3cm}, clip]{figures/diff_exm.pdf}
    \label{fig:iso_exmaple2}
    }  
    \caption{The tree rooted at node 1 in the source space is isomorphic to the target tree when specific edges, marked in red, are properly connected or disconnected.}
    \label{fig:iso_exmaple}
\end{figure}




% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth, page=2, trim={0 2.5cm 0 3cm}, clip]{figures/diff_exm.pdf}
%     \caption{An example of generating  propositional Boolean variables are generated from three different sources:  1)}
%     \label{fig:encode_exm}
% \end{figure}




\textbf{The deducing phase} In this phase, our objective is to derive low-level edit scripts from SAT solutions. These low-level edit scripts act as an intermediate layer between the solutions and the resulting high-level edit scripts and can be constructed by three distinct \textit{atomic} edit actions: \texttt{dcon}, \texttt{del} and \texttt{con}. Importantly, these atomic edit actions can be easily inferred from SAT solutions. Let's consider some examples to illustrate how the atomic edit actions can be inferred from SAT solutions.

\begin{itemize}
    \item In the case where $\evar{2}{1}{4} = 0$ and $\mvar{4}{18} = 1 $, it indicates that the existing edge $\fe{2}{1}$ (interpreted as the edge $e_1$ or the first child slot of the parent node 2) is available or $free$, and node 4 needs to be reused later due to a matching literal being true. Consequently, we can infer the corresponding atomic edit action as $\dcon{2}{1}{4}$.
    \item Now, let's examine another scenario where $\evar{3}{2}{7}= 0$
    and no match variables are true for node 7. In this situation, it suggests that the sub-tree rooted at node 7 should be deleted. Thus, the inferred atomic edit action would be $\del{3}{2}{7}$.
    \item Lastly, suppose we have the SAT solution where $\evar{3}{2}{4}= 1$, indicating that node 4 is now connected to node 3 via edge $\fe{3}{2}$. This implies that a connection between these nodes exists, leading to the derived atomic edit action of $\con{3}{2}{4}$.
\end{itemize}

While it may appear relatively straightforward to deduce atomic actions from SAT solutions, generating low-level edit scripts using these actions poses a challenge. This challenge arises due to the fact that, from the solver's perspective, all modifications to the edge configuration occur simultaneously. Indeed, failing to specify the correct order of edit actions can give rise to various issues. To illustrate this point, let's consider a scenario where the action $\con{2}{1}{21}$ is performed before the action $\dcon{2}{1}{4}$. In this case, the first child position $\fe{2}{1}$ is already occupied by node 4. Consequently, it would not make sense to connect node 21 to node 2 via $\fe{2}{1}$ since it is already in use. 


However, there is a simple strategy to ensure the correct ordering: perform the \texttt{dcon} actions first, followed by the \texttt{del} actions, and finally the \texttt{con} actions. The underlying intuition is as follows: when executing \texttt{dcon} actions, a pair of $free$ edges and nodes is created. The objective is to maximize the number of these pairs. Subsequently, the \texttt{del} actions exclusively add $free$ edges. Lastly, the \texttt{con} actions reduce the number of $free$ edges and nodes by diminishing a pair. Table \ref{tab:atomic_ordering} illustrates a concrete example. Furthermore, it is important to highlight that our atomic actions, as well as low-level edit scripts, maintain type safety through detailed tracking of edges and nodes. We will delve into further details about this phase in Section \ref{sec:phase2}.
% If we were to swap the order of the actions, the issue would be resolved, and the edit actions would be applied correctly without conflicts. 
% More interest
% \jl{update attri}
\begin{table}
\begin{tabular}{lccc}
  \hline
      High-level Actions ($\overline{\Delta}$)  & Atomic Actions ($\underline{\Delta}$) & \textit{Free} Node ($\accentset{\circ}{N}$)  & \textit{Free} Edge ($\accentset{\circ}{E}$)  \\
  \hline
  \hline
  
   &  & 21,22 &  $\emptyset$  \\
  \hline
   $\Del{3}{2}{7}$ & $\del{3}{2}{7}$ &   21,22 & $\fe{3}{2}$   \\
  \hline
  
    \multirow{2}{*}{$\Mov{4}{2}{1}{3}{2}$} &$\dcon{2}{1}{4}$  & 21,22,4 & $\fe{2}{1}$, $\fe{3}{2}$   \\
    & $\con{3}{2}{4}$ & 21,22 & $\fe{2}{1}$ \\
    \hline
  $\Ins{2}{1}{21}$ & $\con{2}{1}{21}$ & 22 & $\emptyset $\\
    \hline
  \multirow{6}{*}{$\texttt{Upd}(5,Add)$} & $\dcon{5}{1}{8}$ & 22,8 & $\fe{5}{1}$  \\
  & $\dcon{5}{2}{9}$ & 22,8,9 & $\fe{5}{1}, \fe{5}{2}$ \\
  & $\del{2}{2}{5}$ & 22,8,9 & $\fe{2}{2}$\\
  & $\con{2}{2}{22}$ & 8,9 & $\fe{22}{1},\fe{22}{2}$ \\
  & $\con{22}{1}{8}$ & 9 & $\fe{22}{2}$ \\
  & $\con{22}{2}{9}$ & $\emptyset$ & $\emptyset$ \\
  \hline
\end{tabular}

\caption{
The low-level edit script, which comprises atomic edit actions and detailed tracking of nodes and edges, ensures both correctness and type safety. The first row of the table indicates the initial state of $free$ nodes and $free$ edges.
% Note we use $((2,e_2),e_1)$ and $((2,e_2),e_2)$ to represent the first and second child position of $(2,e_2)$ --- the second child position of node 2 after deleting node 5. Later, when node 22 occupies the second child position of node 2, $((2,e_2),e_1)$ and $((2,e_2),e_2)$ becomes $(22,e_1)$ and $(22,e_2)$. 
}
\vspace{-20pt}
\label{tab:atomic_ordering}

\end{table}
% Informally, \emph{$connect(n, n_p, e_i)$} and  \emph{$disconnect(n, n_p, e_i)$} disconnect and connect nodes $n$ and $n_p$ via edge $e_i$; \emph{$delete(n, n_p, e_i)$} deletes subtree rooted at node $n$ while \emph{$disconnect(n, n_p, e_i)$} only detaches that subtree so it can be used later.  Formal definition and semantics of these atomic edit actions will be introduced in Section \ref{sec:phase2}.
% By examining the SAT solution, particularly the assignment to edge variables, we can gain a clear understanding of the changes that occurred in the source tree. This understanding is achieved by employing three distinct \textit{atomic} edit actions: \emph{disconnect}, \emph{delete} and \emph{connect} that manipulate the configuration of edges. 
% Informally, \emph{$connect(n, n_p, e_i)$} and  \emph{$disconnect(n, n_p, e_i)$} disconnect and connect nodes $n$ and $n_p$ via edge $e_i$; \emph{$delete(n, n_p, e_i)$} deletes subtree rooted at node $n$ while \emph{$disconnect(n, n_p, e_i)$} only detaches that subtree so it can be used later. Formal definition and semantics of these atomic edit actions will be introduced in Section \ref{sec:phase2}.
% \begin{figure}[h]
%     \centering
%     \includegraphics[page=4, width=0.9\textwidth,trim={0 0cm 0 3cm}, clip]{figures/diff_exm.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% \hy{add swap}

\textbf{The synthesizing phase} During this phase, we generate high-level edit scripts by synthesizing high-level edit actions, such as \texttt{Upd}, \texttt{Ins}, \texttt{Del}, and \texttt{Mov} from low-level edit scripts. Let's consider some examples to illustrate how to synthesize high-level edit actions from atomic edit actions:

\begin{itemize}
    \item The $\dcon{2}{1}{4}$ atomic action $frees$
    node 4 and edge $\fe{2}{1}$, and $\del{3}{2}{7}$ atomic action $frees$
    edge $\fe{3}{2}$, whereas $\con{3}{2}{4}$ requires the usage of node 4 and edge $\fe{3}{2}$. Since node 4 is detached and reattached to a new position, we identify this as a move action $\Mov{4}{2}{1}{3}{2}$. The $\Del{3}{2}{7}$ action also serves as a high-level operation and should appear before $\Mov{4}{2}{1}{3}{2}$. 

    \item Following previous process, we now have edge $\halfe{2}{1}$ $free$. And the $\con{2}{2}{21}$, requires the usage of edge $\fe{2}{1}$ and virtual node 21. Such a connection involves a virtual node that corresponds to an insert action $\Ins{2}{1}{21}$.

    \item The actions $\dcon{5}{1}{8}$ and $\dcon{5}{2}{9}$ $free$ nodes 8 and 9, as well as edges $\fe{5}{1}$ and $\fe{5}{2}$. Subsequently, the action $\del{2}{2}{5}$ removes node 5 and $frees$ the edge $\fe{2}{2}$, which is later utilized by the action $\con{2}{2}{22}$. The actions $\con{22}{1}{8}$ and $\con{22}{2}{9}$ establish connections between the edges and the new node 22, effectively replacing node 5. In essence, these actions update the internal nodes without modifying their children, which can be interpreted as an update action $\texttt{Upd}(5,Add)$.
\end{itemize}

    % ($(5,e_1)$ and $(5,e_2)$ becomes $((2,e_2),e_1)$ and $((2,e_2),e_2)$); then $connect(22,2,e_2)$ requires using $(2,e_2)$ and virtual node 22, thus applying $connect(22,2,e_2)$ rename edges $((2,e_2),e_1)$ and $((2,e_2),e_2)$) to  $((22,e_1)$ and $(22,e_2)$), which then demands by $connect(8,22,e_1)$ and $connect(9,22,e_2)$.

As we can observe, synthesizing high-level actions can be significantly more challenging than deducing low-level edit scripts due to the presence of complex dependencies. To overcome this challenge, we leverage topological ordering and detailed tracking of nodes and edges to synthesize high-level actions in the correct order. Figure \ref{fig:topo_example} illustrates the dependency graph of low-level edits and how they form high-level edit actions following a topological order of the dependency graph. The two disconnected subgraphs imply their independence from each other, thereby rendering their execution order inconsequential. Within each subgraph, we synthesize the high-level actions following some rigorous semantics and type rules. Additional details and formal analysis on the type safety, semantics, and other aspects of high-level edit scripts will be provided in Section \ref{sec:phase3}. 

% From our definition, \emph{del} is the same as how we do \emph{delete} while \emph{insert}




% To overcome this challenge, we employ a strategy that involves detailed tracking of edges and nodes, as well as the use of topological ordering. By meticulously tracking the specific edges and nodes affected by each edit action, we can ensure that the edit actions are applied in a logical and meaningful sequence. 


\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth, trim={0 3cm 0 3.5cm}, clip]{figures/topo.pdf} 
    
    \caption{Dependency graph of atomic edits of the example in Figure \ref{fig:overview_sat}. The dashed regions are merged high-level edits, which form following a topological order of the dependency graph.}
    \label{fig:topo_example}
\end{figure}




% \allen{Change the name of tree reducer}
% To make the tree differencing problem more tractable, the input AST is first transformed into a reduced tree format that keeps only the minimum information needed for further processing. This reduced tree format reduces the size and complexity of the problem, making it easier to solve. The reduced tree format aims to 

% is designed independent of language-specific grammar and rules. 

% Another advantage of the {\satdiff} framework is that it is language-independent. Because the input to the framework is an abstract syntax tree, the framework can be used with any programming language that has an abstract syntax tree representation. This means that the {\satdiff} framework is a highly adaptable and flexible approach that can be applied to a wide range of programming languages and scenarios.









% Once the reduced tree format is obtained, an encoder is used to specify both hard and soft constraints. 


% The hard constraints are rules that must be satisfied to ensure that the edit script is valid, while the soft constraints are rules that aim to find the optimal edit script. The encoder takes these constraints and generates a {\Large M}AX{\Large S}AT problem that can be solved by an off-the-shelf {\Large M}AX{\Large S}AT solver.

% The {\Large M}AX{\Large S}AT solver determines a minimum subset of soft constraints that need to be violated to satisfy the hard constraints and optimize the edit script. Finally, a decoder interprets the violation of these soft constraints and generates a sequence of edit operations, which represents the differences between the two ASTs. This sequence of edit operations is the edit script that is output by the {\satdiff} framework. One key 


% Finally, the {\satdiff} framework is highly efficient. By transforming the tree differencing problem into a {\Large M}AX{\Large S}AT problem and using an off-the-shelf {\Large M}AX{\Large S}AT solver, the framework can find the optimal edit script quickly and with minimal computational overhead. This efficiency makes the {\satdiff} framework an ideal solution for time-sensitive applications and large-scale tree differencing tasks.

% \textcolor{red}{Say something about the advantages.}
% Another advantage of the {\satdiff} framework is that it is language-independent. Because the input to the framework is an abstract syntax tree, the framework can be used with any programming language that has an abstract syntax tree representation. This means that the {\satdiff} framework is a highly adaptable and flexible approach that can be applied to a wide range of programming languages and scenarios.

% The {\satdiff} framework is also highly customizable, allowing users to specify their own hard and soft constraints. This customization enables users to tailor the framework to their specific needs and optimize the edit script for their particular use case.


% In summary, the {\satdiff} framework is a powerful approach to tree differencing that leverages the power of {\Large M}AX{\Large S}AT solvers to efficiently find the optimal edit script. It is a flexible and adaptable approach that can be applied to a wide range of programming languages and scenarios.



==> related_1.tex <==
\section{Related work}
\label{sec:related}
% In this section, we present the related work on code differencing, from text to graph granularity.

The process of computing differences between two versions of a source file can be performed at different levels of granularity, ranging from textual comparisons to more sophisticated analyses based on code tree structures. Textual-level differencing techniques are the most commonly used. For instance, the Unix {\fontfamily{cmss}\selectfont diff} utility holds a central role in numerous modern distributed version control systems, including popular platforms like Git, Mercurial, and Darcs. It employs the Myers algorithm \cite{DBLP:journals/algorithmica/Meyers86} to compare two versions of a source code file and identify the added or deleted lines. These line-by-line algorithms, based on such granularity, are generally fast and language-independent. However, such methods have two significant limitations. Firstly, they generate an edit script that solely captures additions and deletions, disregarding other types of edit actions such as updates and moves. Secondly, they operate at a coarse-grained level of granularity compared to the abstract syntax tree (AST), which fails to align with the structural organization of the source code.

To address these limitations, tree/structural diffing approaches have been introduced, which operate at the AST level. These algorithms offer a significant advantage as they generate edit scripts that are aware of the tree structure of the code. This awareness enables more comprehensive and nuanced comparisons, encompassing structural modifications within the code, such as actions involving the addition, deletion, and updating of nodes. By considering these structural changes, the tree diffing approaches provide a more thorough analysis of the code differences, capturing a wider range of edit actions and providing a deeper understanding of the code evolution between versions. One pioneering work in this line of research was proposed by Chawathe et al. The approach begins by identifying matching nodes between the source and target trees through heuristics that assess their similarity. Once the matching nodes are established, an optimal edit script is derived, comprising operations such as insertions, deletions, moves, and updates. The original heuristics proposed by Chawathe et al. are specifically optimized for comparing flatly structured documents like LaTeX files. Since then, most tree-diffing approaches have adhered to the same paradigm but employed different similarity metrics for node matching. 

% \vspace{-5 pt}

ChangeDistiller \cite{ChangeDistilling} utilizes a bigram string similarity measure and inner node similarity weighting to improve node matching on fine-grained syntax trees. In contrast, GumTree \cite{gumtree} employs a top-down greedy search to identify the largest isomorphic subtrees between the source and target trees, enabling fine-grained differencing of Java ASTs. Additionally, JSync \cite{JSync} introduces characteristic vectors for measuring structural similarity between (sub)trees and uses heuristics to identify highly similar pairs as clones, facilitating clone detection in JavaScript. Furthermore, X-Diff \cite{XDiff} designs node signatures as the primary criterion for node matching and presents an effective algorithm that combines XML structure characteristics with standard tree diffing techniques. MTDIFF \cite{MTDIFF} incorporates several optimizations for identifying unchanged code, mapping inner nodes, and other processes. These optimizations result in improved accuracy when detecting code movements. 

Additionally, there is a line of work \cite{MTDIFF,hdiff,truediff} that adopts a different strategy for searching node matching, leveraging hashmaps instead of the similarity scores paradigm as seen in \cite{ChawatheRGW96}. 
More specifically, they compute a unique cryptographic hash for each subtree, and matches are found if and only if two subtrees' hashes are equal. While hashmap methods are more efficient compared to similarity-based methods, which often have a quadratic running time, it is important to note that finding mapping pairs based on the same hash value imposes a more restricted condition. This condition may underestimate the potential matched nodes, thereby limiting the effectiveness of the approach. In contrast, our proposed approach, {\satdiff}, is novel as it does not rely on heuristics. The encoding of {\satdiff} allows exhaustive search on node matching, making it capable of providing an optimal edit script compared to heuristics-based approaches. 

There is also a line of work focused on achieving type safety in addressing the tree diffing problem.\cite{truediff} highlight the type safety issues present in existing solutions, such as \textit{Gumtree} \cite{gumtree}. Specifically, these issues arise when intermediate trees become ill-typed during the execution of the generated edit script. For example, a move operation that connects a subtree to its new parent may result in the new parent having more children than specified by its defined type. They further argue that this limitation poses a significant obstacle to patching typed tree representations, including algebraic data types. It is worth mentioning that our {\satdiff} approach achieves type safety, which is guaranteed by our constraint encoding. Furthermore, we can perform type checks and track the execution of edit scripts based on the type system of edit operations. Our theoretical analysis also suggests that our edit scripts are type safe.



% Fluri et al. [7] introduced heuristics based on statistical metrics, aiming to enhance node matching on generic syntax trees.
% Falleri et al. [6] optimized these heuristics specifically for fine-grained differencing of Java Abstract Syntax Trees (ASTs) in the GumTree tool.
% Nguyen et al. [14] tailored the heuristics to clone detection in JavaScript, taking into account the specific characteristics of that language.
% Dotzler and Philippsen [5] proposed several optimizations applicable to all the aforementioned approaches. Notably, they introduced a move optimization technique that utilizes cryptographic hashes to identify isomorphic subtrees efficiently. 



% These different heuristics and optimizations contribute to advancing the field of tree-diffing and enable more accurate and context-specific comparisons of source code.








































% Introduction:
% Tree differencing is a fundamental task in software engineering, and it is commonly used in version control systems, program analysis, and debugging. Several tree differencing algorithms have been proposed in the literature. In this paper, we review some of the most relevant works in this area.

% \textcolor{magenta}{need categorization.}

% GumTree:
% GumTree \cite{DBLP:conf/kbse/FalleriMBMM14} is a tree-based differencing algorithm proposed by Falleri et al. in 2014. It is designed to work with Abstract Syntax Trees (ASTs) and uses a hierarchical differencing approach. The algorithm first constructs a mapping between the nodes of the two trees and then computes the differences between the mapped nodes. GumTree has been evaluated on various software artifacts, and the results show that it outperforms other tree-based differencing algorithms in terms of accuracy and speed.

% Change Distilling:
% Change Distilling \cite{DBLP:journals/tse/FluriWPG07} is another tree-based differencing algorithm proposed by Fluri et al. in 2007. It improves the existing algorithm by Chawathe et al. for extracting changes in hierarchically structured data. It works by finding both a match between the nodes of the compared two abstract syntax trees and a minimum edit script that can transform one tree into the other given the computed matching. The method achieved significant improvements in extracting types of source code changes and it reaches a mean absolute percentage error of 34 percent, compared to the 79 percent reached by the original algorithm by Chawathe et al \cite{DBLP:conf/sigmod/ChawatheRGW96}.


% TopDiff:
% TopDiff algorithm \cite{DBLP:conf/cikm/0001A20}, created by Pawlik and Augsten, is inpired by the algorithm by Touzet. It is a new tree edit distance algorithm that is linear in the tree size for similar trees. The algorithm leverages
% the similarity of two tree versions to scale the diff computation to
% large trees. And the new concept of top node pairs is introduced to avoid redundant distance computations, making the algorithm efficient for large and flat trees.

% X-tree Diff+:
% X-tree Diff+ \cite{DBLP:conf/euc/LeeK06}, based on X-tree Diff, is an efficient change detection algorithm for tree-structured documents such as HTML, XML documents. In this algorithm, difference (change) between documents can be viewed as a sequence of edit operations. Tuning and copy operation increase matching ratio drastically, which allows X-tree Diff+ to produce better quality of edit scripts and runs fast equivalent to the time complexity of fastest heuristic algorithms.

% DECKARD:
% DECKARD is a novel algorithm proposed by Jiang et al. in 2007 for detecting similar trees and a practical implementation for detecting code clones \cite{DBLP:conf/icse/JiangMSG07}. The main idea of the algorithm is to compute certain characteristic vectors to approximate structural information within ASTs and then adapt Locality Sensitive Hashing (LSH) \cite{DBLP:conf/compgeom/DatarIIM04} to efficiently cluster similar vectors (and thus code clones). Through evaluation on large code bases written in C and Java including the Linux kernel and JDK, DECKARD is shown to be both scalable and accurate. It is also language independent, applicable to any language with a formally specified grammar as well.

% RTED:
% RTED is developed by Pawlik and Augsten \cite{DBLP:journals/corr/abs-1201-0230}. It is an efficient algorithm for computing the optimal LRH strategy for GTED. This algorithm adopts a decomposition strategy which recursively decomposes the input trees into subforests by removing nodes. RTED requires $O(n^2)$ space as the
% most space-efficient competitors, and its runtime complexity of $O(n^3)$ in the worst case is optimal.

% PMatch:
% PMatch is propsed by Lang et al. and it is a method based on code semantic similarity to detect the patched binary functions. PMatch achieves an 86.43\% average accuracy in detecting the patched functions, which outperforms the state-of-the-art work, and costs only 65.14ms per function. Besides, at the $O^3$ high optimization level, PMatch achieves an accuracy improvement of over 20%.


% Conclusion:
% In this paper, we reviewed some of the most relevant tree differencing algorithms in the literature. GumTree, \textcolor{magenta}{and some real algorithms} are some of the most widely used algorithms in this area. While these algorithms have different approaches, they all aim to compute the differences between two trees efficiently and accurately. The choice of a tree differencing algorithm depends on the specific application and the characteristics of the input data.

